Suitably graded THB-spline refinement and coarsening: Towards an adaptive isogeometric analysis of additive manufacturing processes

In the present work we introduce a complete set of algorithms to efficiently perform adaptive refinement and coarsening by exploiting truncated hierarchical B-splines (THB-splines) defined on suitably graded isogeometric meshes, that are called admissible mesh configurations. We apply the proposed algorithms to two-dimensional linear heat transfer problems with localized moving heat source, as simplified models for additive manufacturing applications. We first verify the accuracy of the admissible adaptive scheme with respect to an overkilled solution, for then comparing our results with similar schemes which consider different refinement and coarsening algorithms, with or without taking into account grading parameters. This study shows that the THB-spline admissible solution delivers an optimal discretization for what concerns not only the accuracy of the approximation, but also the (reduced) number of degrees of freedom per time step. In the last example we investigate the capability of the algorithms to approximate the thermal history of the problem for a more complicated source path. The comparison with uniform and non-admissible hierarchical meshes demonstrates that also in this case our adaptive scheme returns the desired accuracy while strongly improving the computational efficiency.

==> general/acknowledgements.tex <==




==> general/journalFooter.tex <==
%\usepackage{fancyhdr}
%\date{}
%\fancypagestyle{plain}{%
%  \renewcommand{\headrulewidth}{0pt}%
%  \fancyhf{}%
%  \fancyfoot[L]{
%  \vspace{-1.25cm} 
%  \footnotesize{Preprint submitted to \textit{\journal{}}  \hfill
%  \publicationDate
%  \\
%  %The final publication is available at
%  % \url{http://link.springer.com/article/10.1007/s00466-014-1118-x} 
%  }} }
